Pool-Party: Exploiting Browser Resource Pools as Side-Channels for Web Tracking

We identify class of covert channels in browsers that are not mitigated by current defenses, which we call "pool-party" attacks. Pool-party attacks allow sites to create covert channels by manipulating limited-but-unpartitioned resource pools. These class of attacks have been known, but in this work we show that they are both more prevalent, more practical for exploitation, and allow exploitation in more ways, than previously identified. These covert channels have sufficient bandwidth to pass cookies and identifiers across site boundaries under practical and real-world conditions. We identify pool-party attacks in all popular browsers, and show they are practical cross-site tracking techniques (i.e., attacks take 0.6s in Chrome and Edge, and 7s in Firefox and Tor Browser). In this paper we make the following contributions: first, we describe pool-party covert channel attacks that exploit limits in application-layer resource pools in browsers. Second, we demonstrate that pool-party attacks are practical, and can be used to track users in all popular browsers; we also share open source implementations of the attack and evaluate them through a representative web crawl. Third, we show that in Gecko based-browsers (including the Tor Browser) pool-party attacks can also be used for cross-profile tracking (e.g., linking user behavior across normal and private browsing sessions). Finally, we discuss possible mitigation strategies and defenses

==> Makefile <==
extensions_to_clean := out aux log bbl blg fls fdb_latexmk glg gls lof glo glsdefs lot toc dvi ist acn acr synctex.gz alg xdy

all: paper

clean:
	@if [[ -f paper.pdf ]]; then \
		rm paper.pdf;\
	fi;
	@for extension in $(extensions_to_clean); do \
		find . -type f -name "*.$$extension" -delete;\
	done;
	@rm -f diff.*

paper:
	latexmk -bibtex -pdf paper
	pdflatex -bibtex -interaction=batchmode paper

diff:
	latexmk -bibtex -pdf diff
	pdflatex -bibtex -interaction=batchmode diff


==> scraps/_2_definition.tex <==
\section{\uTechniqueName{} Definition and Background}
\label{sec:definitions}
In this section we provide the background context for how \TechniqueName{} attacks
relate to other \Web{} tracking techniques in general, and other methods of
creating browser side-channels in particular. We also describe why existing browser protections
fail to protect users against \TechniqueName{} attacks.

This section proceeds
by first defining what \Web{} tracking is, then describes how websites can
track users using \TechniqueName{} attacks. Next, we describe
how \TechniqueName{} attacks relate to both i) other side-channels in browsers,
and ii) conventional \Web{} tracking techniques.  We follow by explaining why 
existing browser protections do not protect users against
\TechniqueName{} attacks, and conclude by describing how
this work relates to a category of attacks previously known to be possible, but not
previously shown to be practical.


\subsection{Web Tracking and Cross-Site Tracking}
\label{sec:definitions:tracking}
This section gives a ``working'' definition of \Web{} tracking. Our goal
in this definition is not to provide a formal, fully unambiguous definition (the
phrase ``\Web{} tracking'' is used too broadly to likely allow for such
a definition), but instead to give a general, practical definition, to build
on throughout the rest of this work.

In this paper, we use the term \Web{} \emph{tracking} to refer to the practice of
the browser-user being re-identified, across conceptual contexts, without the
user's consent. We use the word \emph{context} broadly, to refer to
the user executing a webpage in such a way that the webpage is not able
to link the users behavior or identity on that page, with the users behavior or
identity on other webpages.

Contexts might be divided by \emph{time} (\EG{} a site
re-identifying a user revisiting the same site a week after first visiting,
despite the user clearing browsing data), \emph{application} (\EG{} a
site re-identifying a user in visiting a site in Safari as the same user
who previously visited the site in Chrome), \emph{profile} (\EG{} a
site identifying that the visiting in an private/incognito browser session
is the same user visiting the site in a standard browser session) or
\emph{sites} (\EG{} two sites colluding to learn that browser sessions
occurring on each site belong to the person). The commonality in all cases
is the users' reasonable expectation that things that happen in one context
are not readily known and available in another context.


\subsection{Description of \uTechniqueName{} Attack}
\label{sec:definitions:pp}
This work presents a new category of side-channels in browsers that we call
\TechniqueName{} attacks. \uTechniqueName{} attacks are side-channels
constructed by two parties manipulating the state of \LBU{} resource pools
to send signals across security or privacy boundaries. Differences
in browser architecture mean that browsers vary in terms of how, and in how
many ways, attackers can carry out \TechniqueName{} attacks, but all popular
browsers are vulnerable at time of this writing.

This section describes how \TechniqueName{} attacks work in general;
Section \ref{sec:eval} gives specific examples of how this category of
attack can be executed in each browser.

\SubPoint{How \uTechniqueName{} Attacks Work}
\uTechniqueName{} attacks work by manipulating pools of browser resources
which are limited (\IE{} the browser restricts how many of the resource websites
can open or consume) and unpartitioned (\IE{} different contexts consume
resources from the same pool). While the examples focused on in this work
utilize \LBU{} pools of network connections, browsers include
many other \LBU{} resource pools that could be similarly exploited, such as
pools of file handles, subprocesses, or other resource handles.

A \TechniqueName{} attack occurs when parties operating in distinct contexts
(contexts the user expects to be distinct and blinded from each other)
intentionally consume and query the availability of the limited resources in
a resource pool, to create a cross-context communication channel. Each context
can then use the communication channel to pass an identifier, allowing each
party to link the users behavior across the two contexts. We note again that
most commonly the two contexts considered here are two different websites running
in the same browser profile, but could also be the same (or different) websites
running in different browser profiles.

\SubPoint{Demonstrative \uTechniqueName{} Attack Example}
\label{sec:definitions:pp:demo}
Again, Section \ref{sec:eval} provides details on specific ways of executing
\TechniqueName{} attacks in popular browsers, but we provide here a simplified
example of how attacks in this category work.

For this toy example, assume a browser vendor wants to improve performance
by only allowing one video element to be loaded at a time, across all sites.
If a video is currently playing on any page, the site will receive an error
if it tries to play a new video.

\input{figures/toy-algo}

Algorithm \ref{algo:toy-algo} presents a toy algorithm where by two
colluding sites can trivially transform this optimization choice into a cross-site tracking mechanism.

While in practice this approach would be slow, we note that it is only provided
to demonstrate the concept, and actual attacks are provided in Section
\ref{sec:eval}. We note three details though: i) the attack works for
any \LBU{} resource, ii) the less common the resource pool'ed feature is on the
\Web{}, the less noisy the channel will be, and iii) the larger the size of the
resource pool, the higher the bandwidth of the resulting communication channel.

\subsection{Relationship to Other Side-Channel Attacks}
\label{sec:definitions:side-channels}
\TechniqueName{} attacks differ from other side-channel attacks by targeting
explicit, intentional, application-imposed limits. This differs from many other
side-channel attacks in two ways, and generally makes \TechniqueName{} attacks
more practical.

First, \TechniqueName{} attacks
target application-level resources, while many other side-channels 
target parts of the system below, or at least distinct from, the
application (\EG{} hardware restrictions like CPU caches,
OS details like interrupt schedules or memory management, or
language runtime features like garbage collection). This is significant because,
the lower in the stack the attacker targets, the more likely it is (all other things
being equal) that the targeted resource will be shared with other actors on the system.
This means that lower-level side-channels are more likely to be noisy, and so more difficult
to communicate over.

Second, related but distinct, \TechniqueName{} attacks target browser-managed
resources, resources that are, in most cases, intentionally shielded from
other applications on the system. This again reduces the chance that
colluding parties will have to contend with a noisy, unpredictable side-channel.


\subsection{Relationship to Other Tracking Methods}
\label{sec:definitions:contrasts}
\TechniqueName{} attacks do not fall neatly into the categories usually used
to describe browser tracking techniques. This subsection briefly describes
the rough-taxonomy used in online-tracking research, and why \TechniqueName{}
does not cleanly fall into existing categories.

\SubPoint{State-full Tracking}
\label{sec:definitions:contrasts:stateful}
``State-full tracking'' most commonly refers to websites using explicit storage APIs
in the Web API (\EG{} cookies, localStorage, indexedDB) to assign identifiers
to browser users, and then read those identifiers back in a different context,
to link the identity (or, browser behavior) across those contexts.

Stateful-tracking also describes other ways websites can set and
read identifiers, by using APIs and browser capabilities not intended for
such purposes. Examples of such techniques include exploiting the browser
HTTP cache, DNS cache or other ways of setting long term state (\EG{} HSTS
instructions~\cite{syverson2018hsts}, favicon caches~\cite{favicon2021}, or,
ironically, storage intended to prevent tracking~\cite{janc2020information}).

\input{tables/browser-partitioning}

Browsers increasingly protect users from stateful tracking by
partitioning storage by context, mostly commonly be the effective-top level
domain (\IE{} \texttt{eTLD+1}) of the website. Giving each context a unique
storage area prevents trackers from reading the same identifier across multiple
contexts, and so prevents the tracker from linking browsing behaviors in
different contexts. Partitioning explicit storage APIs is often referred to
as \textbf{DOM Storage} partitioning.  Partitioning caches and other ``incidental''
ways sites can store values is often called \textbf{network state partitioning}.
Table \ref{table:browser-partitioning} provides a summary of state partitioning
in popular browsers.

Browser state partitioning strategies fail to defend against \TechniqueName{}
attacks because \TechniqueName{} attacks do not rely on setting or retrieving
browser state (at least not in the way state is generally discussed in this
context, meaning the ways that sites can write state to the users profile).
\uTechniqueName{} attacks instead rely on implementation details of browser
architecture, where device resources are \LBU{}. While partitioning strategies
could also be used to defend against \TechniqueName{} attacks, as discussed in
Section \ref{sec:discussion}, certain aspects of these attacks make partitioning
approaches difficult in practice.

\SubPoint{Note on Chromium Partitioning Features}
All analysis in this work uses a hardened, non-default configuration of Chromium
browsers. First, we disable third-party storage (\IE{} block third party cookies). Second, we enable Chromium's network partitioning features.  These features,
which are not enabled by default for most Chrome and Edge users are referred to generally as \texttt{``\NIK{}''}
(NIK)~\footnote{\url{https://github.com/shivanigithub/http-cache-partitioning\#choosing-the-partitioning-key}}.
When enabled, the \NIK{} feature causes Chromium to partition network state by top level eTLD+1\footnote{Chromium's \NIK{}
actually employs a more complex system for determining the appropriate cache
key for a resource than just the top level frame's eTLD+1, but for all purposes
relevant to this paper, the system can be simplified to
``top level frame's eTLD+1'' without error.}, in a
manner similar to, but not quite as comprehensive as, Gecko based
browsers. Importantly, the \NIK{} system partitions network state, but not DOM
storage.

By default, \NIK{} features are disabled in Chrome and Edge, though
they are enabled for a small percentage of users as part of ongoing
performance tests. Brave Browser, which is also built on Chromium,
enables the \NIK{} system for all users.

We choose to disable third-party state and enable the \NIK{} features in Chromium to demonstrate that Chromium-based browsers are vulnerable
to \TechniqueName{} attacks, even in highly hardened configurations.


\SubPoint{Stateless Tracking}
\label{sec:definitions:contrasts:stateless}
``Stateless tracking,'' (also often called ``browser fingerprinting'') refers to
the category of \Web{} tracking techniques whereby the attacker constructs a
unique identifier for the user by combining a large number of
semi-distinguishing browser and environmental attributes into a stable, unique identifier. Examples of such semi-distinguishing features include the operating system the browser is running on, the browser version, the names and the number of plugins or hardware devices available, and the details around the graphics
and audio hardware present, among many others~\cite{laperdrix2020browser}.

In contrast to ``state-ful'' tracking techniques, ``stateless''
techniques do not require sites to be able to set and read identifiers across
context boundaries, and so are robust to storage partitioning defenses.
Stateless attacks instead rely on three conditions to be successful:

\begin{enumerate}
  \item \textbf{Coordination:} code running in different contexts must know
    to query the same (or at least sufficiently large intersection of) browser
    attributes.
  \item \textbf{Stability:} the browser must present the same values for the
    same semi-distinguishing attributes across contexts (otherwise the browser
    will yield different fingerprints in different contexts, preventing
    the attacker from matching the two fingerprints).
  \item \textbf{Uniqueness:} the browser must present enough semi-distinguishing attributes to allow the site to accurately
    differentiate between users (otherwise the attack will confuse two
    different users as the same person)
\end{enumerate}

\input{tables/fingerprinting-defenses}

Browsers defend against ``stateless'' trackers by attacking any of these
three requirements. A browser might prevent \textbf{coordination} by blocking
fingerprinting code on sites, or prevent \textbf{stability} by making the
browser present different attributes to different sites (such as in
\cite{laperdrix2017fprandom, nikiforakis2015privaricator}), or prevent
\textbf{uniqueness} by reducing the entropy provided by each attribute. Table
\ref{table:fingerprinting-defenses} provides a summary of deployed
``stateless'' defenses in popular browsers.

Browser defenses against ``stateless'' tracking techniques fail to defend
against \TechniqueName{} attacks because of differences in the nature of the
attack. ``Stateless'' techniques target stable semi-distinguishing browser
characteristics which are set by a page's execution environment.
\uTechniqueName{} attacks, in contrast, are enabled by sites consuming
and reading the availability of limited resources in the browser across
execution contexts. Therefore, unsurprisingly, browser defenses against
``stateless'' tracking provide no protection against \TechniqueName{} attacks.


\SubPoint{XS (Cross-Site) Leaks}
\uTechniqueName{} attacks are most similar to a category of attack loosely
called ``XSLeaks''~\footnote{\url{https://xsleaks.dev/}}, a broad collection of
ways sites can send signals to each other in ways generally unintended by
browser vendors. However, we note that in contrast to ``state-ful'',
``stateless,'' \TechniqueName{} attacks, XSLeaks do not have a common cause
or remedy; instead, XSLeaks can be largely thought of as a catchall
for cross-site (or cross-context) techniques that do not not fit in another
category. Examples of XSLeaks include timing channels stemming from a variety of
causes, unintended side effects of experimental browser
features~\footnote{\EG{} \url{https://xsleaks.dev/docs/attacks/experiments/scroll-to-text-fragment/}},
or misuse of other browser APIs~\footnote{\EG{} \url{https://xsleaks.dev/docs/attacks/window-references/}}.

The lack of a common cause of XSLeaks makes it impossible to generalize about
defensive strategies or deployed browser defenses. Recent work in this area has 
identified ways sites can leak information across browser-imposed boundaries,
including through unintended side effects in how browsers handle errors, implement
cross-origin opener-policy (COOP)~\footnote{\url{https://developer.mozilla.org/en-US/docs/Web/HTTP/Headers/Cross-Origin-Opener-Policy}}, cross-origin resource policy
(CORP)~\footnote{\url{https://developer.mozilla.org/en-US/docs/Web/HTTP/Cross-Origin_Resource_Policy_(CORP)}},
and cross-origin read blocking (CORB)~\footnote{\url{https://fetch.spec.whatwg.org/\#corb}} policies,
or limit the length of redirection chains, among many other signals~\cite{knittel2021xsinator}.

We note though that \TechniqueName{} attacks are most common to the ``connection
pool'' attacks identified by the XSLeaks
project~\footnote{\url{https://xsleaks.dev/docs/attacks/timing-attacks/connection-pool/}}.
This work makes the following contributions beyond the issues documented
by the XSLeaks project, and the related work done by Kinttel \EtAl{}~\cite{knittel2021xsinator}.

\textbf{First}, this work identifies and defines a larger category of attack,
where by any \LBU{} resource pool can be transformed into a side-channel (and
so, a tracking technique).
The connection pools attack documented by the XSLeaks project is 
a subset of the larger category of attack discussed in this work.
While \LBU{} connection pools can be used to conduct \TechniqueName{} attacks,
\TechniqueName{} attacks can also be carried out in other browser resource pool
(\EG{} resource handles, subprocess pools, etc). Section~\ref{sec:discussion:additional}
identifies resource pools in browsers that can be exploited for \TechniqueName{} attacks 
that are not connection pools.

\textbf{Second}, we demonstrate that attacks of this type are not just theoretically
possible, but are practical, and are real-world threats to \Web{} privacy.

\textbf{Third}, the presented ``connection pool'' attack relies on abusing the connection pool
to create timing channels, while \TechniqueName{} attacks utilize the number of
available resources in the pool to create the
communication channel. This seemingly-small difference is significant. Using
the amount of availability of resources in the pool as the communication channel
makes the attack more robust to noise introduced from other sites, and means that
mitigations against one form of the attack may not apply to the other.

==> scraps/_prev_1_introduction.tex <==
\section{Introduction}
\label{sec:intro}

Cross-site tracking is a common and well-studied problem on the \Web{}. Cross-site tracking refers to a situation where one party (the tracker) is able to link a \Web{}-user's activities
across multiple sites. Cross-site tracking allows trackers to
build profiles of \Web{} users' interests, infer and share information
about individuals the \Web{} user might not have intended to share, or
inflict any of the other kinds of harms extensively discussed in existing privacy
research.

At root, cross-site trackers create a unique identifier for each \Web{} user,
and use that to re-identify an individual across distinct contexts. These
identifiers must be both \emph{unique} (otherwise the identifier would not be useful
for distinguishing users from each other) and \emph{reusable} (otherwise
the identifier wouldn't be useful for linking activities). These identifiers
can either be set through browser APIs (\EG{} setting and resending a third-party
cookie), passively derived (\EG{} browser fingerprinting), or
explicitly provided by the user (\EG{} an email-address or user-name reused across sites).

A wide range of approaches have been tried to prevent
trackers from creating and/or reading unique identifiers for users. Content
blockers and filter lists identify trackers and prevent them from operating
in each context. Blocking \TPS{} removes the browser capability
most commonly used for re-identifying users across contexts. Other tools
aim to remove or modify browser APIs to reduce the identifiability
of browser fingerprinting techniques.

While each of these approaches have proven useful, each also has
limitations that prevents them from either being widely deployed in browsers,
from being a comprehensive protection, or both. Filter lists, for example,
have coverage issues, and can be evaded by determined trackers\cite{chen2021detecting}. Blocking
all \TPS{} can break websites that integrate with \TPs{} for benign or user
serving purposes (for example, a site that wishes to integrate with a \TP{} single sign-on provider). And disabling the features trackers use to ``fingerprint''
browsers can also break desirable page behaviors (as discussed in ~\cite{iqbal2021fingerprinting}).


In response, privacy-focused browsers have adopted \emph{``partitioning''} as
tracking defense strategy. 
Partitioning prevents cross-site tracking by
preventing the reuse of identifiers across contexts. Partitioning
aims to prevent \CST{} by providing \TPs{} with different resources
for each context the \TP{} operates in, denying the \TP{} a common identifier
to link user with across contexts.
Partitioning strategies are appealing because they are general (\IE{}
they do not rely on identifying bad-actors) and compatible (\IE{} \TPs{}
have access to the same APIs they had access to pre-partitioning).

As a result, all three of the main browser engines have included partitioning
features. WebKit (used in Safari) partitions DOM storage and some kinds of
network state, Gecko (used in Firefox and the Tor Browser Bundle) partition
DOM storage and network state, and Chromium (used in Chrome, Edge, Brave) partitions
network state\footnote{At time of writing, network state partitioning is being
tested for a portion of Chrome users, as part of the engine's ``NetworkIsolationKey''
feature}. Brave has extended Chromium to also partition \TP{}.

In this work we show that the partitioning strategies in all major browsers
are incomplete, and that \TP{} trackers can circumvent these protections
to re-enable the kinds of tracking partitioning was designed to prevent.
While such circumventions have been known to be theoretically possible,
we show that such attacks are practical, reliable, and exploitable using
capabilities available to traditional tracking scripts. We show that our
technique can be used to bypass the privacy-protections intended by
partitioning in all popular browsers and browser engines, even when
each browsers' anti-tracking features are enabled and hardened, and even in
privacy-focused browsers (\EG{} Tor Browser Bundle and Brave Browser). Finally,
we show that our partitioning-circumvention technique can be leveraged to
not only track users across sites, but in some browser engines (\IE{} Gecko)
the technique can be used to identify people across profiles, such as across
private browsing or incognito mode sessions.

Our attack approach, which we call \TechniqueName{}, relies of
\LBU{} resource pools in the browser as a coordination
mechanism, where the same, or colluding, third-parties can use
contention in the resource pool as a communication channel. \uTPs{} can
then use such communication channels to communicate across partitions,
allowing the \TP{} to re-identify the user across contexts, and so continue
tracking as if the partitioning features were not in place.

We demonstrate our attack through the \LBU{} resource
pools provided by network-channels in each browser. We note though that
our attack approach is generic to any \LBU{} resource pool, which could take
the form of available file handles or system processes. The larger the
\LBU{} pool, the higher bandwidth and more stable the communication
channel is.

In Chromium and WebKit, the resource-pools we use to demonstrate our attack in
are shared per browser profile, meaning that \TPs{} operating on any page
within a browser profile can communicate with each other. In Gecko though,
the resource-pools we target are application-wide, and so shared across all
profiles. This has the significant implication that pages operating across
profiles can communicate with each other. In practice this means that
a page operating in a private browsing window can communicate with a page
running in a ``normal'' browsing session, allowing a tracker to link your
intended-private behaviors with your normal browsing activities.

\subsection{Contributions}

More formally, in this work we make the following contributions:

\begin{enumerate}
    \item We \textbf{define a category of practical cross site-tracking technique} which
        we refer to as ``\TechniqueName{} attacks'', and describe how the approach differs
        from the kinds of privacy attacks browsers currently aim to defend against;
    \item We \textbf{empirically evaluate \TechniqueName{}} as an attack category,
        and demonstrate that all popular browsers and browser engines are
        vulnerable to forms of the attack;
    \item We provide two \textbf{open-source, proof-of-concept} implementations of
        our attack that work in all browsers~\footnote{\SourceLink{}};
    \item We perform a \textbf{web-scale measurement} to evaluate the availability,
        bandwidth, and stability of \TechniqueName{} attacks, and find
        that attacks are practical in all current browser;
    \item We \textbf{discuss potential mitigation strategies} for how browsers
        could harden themselves against \TechniqueName{} attacks.
\end{enumerate}

\subsection{Responsible Disclosure}
We have presented our findings to the following browser vendors
(in alphabetical order): Brave, Google, Microsoft, Mozilla, Opera, Tor
Project. All reports were made over 90 days in advance of this submission,
as per the IEEE ``Ethical Considerations for Vulnerability Disclosure''
guidelines. Microsoft and Opera responded that since the discussed vulnerabilities
were in Chromium, they would wait for Google to address the problem. The Tor
Project similarly said they would rely on Mozilla addressing the
vulnerabilities.

We are in ongoing discussion with the Brave, Google, and Mozilla
security teams regarding the vulnerabilities identified in this work. All
three browser vendors have filed related security bug reports and have expressed
intent to address these leaks.

All three organizations were made aware of this submission, and were provided with
pre-print versions of this paper.

==> scraps/algo.tex <==
% \begin{enumerate}
%   \item \textbf{Site A} generates a unique identifier for the user, stores
%     it in a cookie, and reports it back to the server.
%   \item If the first bit of the identifier is 1 or 0, \textbf{Site A} does
%     or doesn't play a video (respectively) for the next 10 seconds.
%   \item \textbf{Site B} tries to play a video. If \textbf{Site B} is able to,
%     it records the first bit of the identifier as 0, and otherwise 1.
%     \textbf{Site B} then waits 10 seconds.
%   \item \textbf{Sites A and B} repeat this process until the entire identifier
%     is transmitted.
%   \item \textbf{Site B} then reports the identifier back to its server, allowing
%     the two servers to link behaviors across the two contexts.
% \end{enumerate}



==> scraps/attack.tex <==
\section{Attack}
\label{sec:attack}
In this section, we describe the covert channels that we create 
by using information leakages in browsers that were
mentioned in section~\ref{BreakingIsolation}. 

\subsection{High-Level Protocol}
\label{sec:highlevel}
This protocol is executed between two parties that do
not know anything about each other. They do not have to start this protocol
at the same time. They just modify and observe the state of a thread pool
to run this protocol. To that end, we designed four steps for this protocol.

\emph{Signal.}
In the first step, they require to start broadcasting a signal
and listening for the signal from the other party. The main goal of this step
is to inform each other that they are ready to begin the protocol. 

\emph{Synchronize.}
Both parties might have data to transfer. In this step, they choose 
who is the first party that send data. Then, the sender prepare itself
for sending data. When it completely prepared, it ask the receiver to start
listening for the data.

\emph{Message Exchange.}
In the third step, the sender splits the data into some packets and sends them one 
by one. In this covert channel, by consuming a specific number of threads, 
the sender sends each packet. On the other hand, for receiving the packets, the 
receiver finds the number of free threads in the thread
pool and infer the value of the packet. 

\emph{Change Roles.}
After sending all the packets, the sender let the receiver know
that all packets are sent. In final step, the receiver gets the
sender role and repeat the \emph{Message Exchange} step.


\subsection{Primitives} 
This protocol works based on the status of the thread pool.
Subsequently, we need to have some functions that modify or
read the status of the tread pool. In this section, we 
describe these functions that are the building blocks of the protocol.

\textbf{Consuming Threads.}
The number of threads that are used by each party, is the base of
this protocol. Each party can use this function, for trying to consume  
a specific number of threads. Using this function, the party either 
consumes the specified number of threads or the thread pool does 
not have that much free threads and it just consumes as much as possible.
Each party knows that how many threads it is currently consumed.

\textbf{Releasing Threads.}
Parties can use this function to release a specific number of threads 
that they have consumed. Thus, using this function one party can 
change the status of the thread pool to transfer some information
to the other party.

\textbf{Wait until the thread pool is Exhausted.}
If one party is required to wait until the other party
consumes all the remaining threads, it can use this function. 
This function tries to use one new thread, if the thread pool assigned a thread, 
it infers that the thread pool is not exhausted yet. 
Thus, it releases the thread and after a short time it repeats trying to use 
one new thread until the thread pool cannot provide any thread.  

\textbf{Wait until the thread pool is available.}
Parties also might need to wait until the other party make the thread
pool available by releasing some threads. 
In this case, they can try to use a new thread and wait until the thread 
pool can provide it. Using this function, the party will be informed that
some threads are free and the thread pool is able to provide new threads.  

\subsection{Details of the protocol} 
In the Protocol~\ref{protocol:ws}, the pseudocode of this covert 
channel is shown. As mentioned in the section~\ref{sec:highlevel}, this 
protocol has four steps. In this section, we describe the details of each step.

\textbf{Signal.} 
In this step, we need to implement two tasks i) sending the signal and 
ii) listening to the signal from the other party. For sending the signal, 
the first party tries to consume 75\% of threads in the 
thread pool. For listening, they wait until the thread pool is exhausted. 
Sending signal from only one party does exhaust the thread pool.
Sometimes later the other party starts this protocol and consumes the rest 
of the threads. At this point, both parties will 
notice that obtaining new threads is not possible anymore, 
that is the signal is received. In other words, they infer the 
presence of the other party. 

\textbf{Synchronize.}
In the second step, they already know that they are ready to start and
they want to choose one party as the sender and the other one 
as the receiver. They make the consensus on the roles based 
on the number of current obtained threads. The party that has consumed 
more than 50\% of threads will be the sender. 
That is, the first party that started the protocol is 
the sender. At this step, the receiver releases all its threads
and the sender consumes all of them. Thus, two parties will notice 
the end of this step by observing that the thread pool is exhausted. 

\textbf{Message Exchange.}
In the third step, parties use the number of free threads to exchange data. 
The sender splits data into packets of $X$ bits and sends packets one by one.
The value of $X$ is depend on the size of the thread pool and can be at most 
$\lfloor\log(poolSize)\rfloor$. For example, if the size of thread pool
is 200, the size of each packet can be equal or less than 7.
At the end of the previous step, the thread pool is exhausted. 
In this step, for sending each packet, it converts the $X$ bits 
into its equivalent decimal number
and releases this number of threads. For example, if it wants
to send 0010010, it releases 18 threads. At this point, the receiver,
which is waiting for the thread pool to become available,
can see that using new threads is possible. Thus, for finding the number of
available threads, it consumes as much as possible threads and 
counts them as the received packet.
For example, if it can consumes 18 threads, it means that it has received
0010010. After receiving this packet, the receiver releases all the
threads and waits for the sender to send the next packet.
When the sender observes that the thread pool is available again, 
it will infer that the packet is delivered. Therefore,
it makes exhausts the thread pool and repeats the mentioned
approach to send the next packet.

When all the packets are sent, the sender releases all its threads. 
In this case, when the receiver tries to consume them, 
it sees that it can obtain more than $2^X+1$ threads.
Because the length of each packet is $X$ bits and the receiver should not be able
to obtain more than $2^X-1$ threads, it can infer that the 
packets are finished and there is no need to wait for other packets.
Thus, at the end of this step, all the threads are consumed by the receiver
and the sender does not have any.

\point{Change roles}
In the \emph{synchronize} step, the first party that started the protocol was selected
as the sender. In this step, the role of the first party will change to receiver.
In this way, the other party can become sender and use the covert channel
to send its data back. After changing their roles, 
they can repeat steps 3 for exchanging data.

\begin{algorithm}
	\floatname{algorithm}{Protocol}
	\caption{Covert Channel using a browser thread pool}
	\label{protocol:ws}
	\textit{Setup.} Parties do not know anything about each other
	and run this separately.
	\sbline
	\textit{Goal.} Parties find each other and share data.
	\sbline
	\textit{The protocol:}
	\begin{enumerate}
		\item \textbf{Signal.}
		\begin{enumerate}
			\item[1] Sending signal: Try to consume 75\% of threads
			\item[2] Listening: Wait until the thread pool is Exhausted
		\end{enumerate}
		
		\item \textbf{Synchronize.} 
		\begin{enumerate}
			\item[1] \textit{if} $($number of consumed threads $>$ 50\%$)\{$
			\item[2] \qquad isSender $\xleftarrow{}$ \textit{true}
			\item[3] \qquad Wait until the thread pool is Available
			\item[4] \qquad consume 100\% of threads
			\item[5] $\}$ \textit{else} $\{$
			\item[6] \qquad isSender $\xleftarrow{}$ \textit{false}
			\item[7] \qquad Release all the threads
			\item[8] \qquad Wait until the thread pool is Exhausted
			\item[9] $\}$
		\end{enumerate}
		
		\item \label{item:msg} \textbf{Message Exchange.}
		\begin{enumerate}
			\item[1] \textit{if} $($isSender$)\{$
			\item[2] \qquad Split data into packets (size=X)
			\item[3] \qquad \textit{for} $($each packet$)\{$
			\item[4] \qquad\qquad \textit{decimal\_num}$\xleftarrow{}$\textit{binaryToDecimal(packet)}
			\item[5] \qquad\qquad Release \textit{decimal\_num} threads
			\item[6] \qquad\qquad Wait until the thread pool is Exhausted
			\item[7] \qquad\qquad Wait until the thread pool is Available
			\item[8] \qquad\qquad consume 100\% of threads
			\item[9] \qquad $\}$
			\item[9] \qquad Release all the threads
			\item[10] $\}$ \textit{else} $\{$
			\item[11] \qquad \textit{while} $($\textit{true}$)\{$
			\item[12] \qquad\qquad Wait until the thread pool is Available
			\item[13] \qquad\qquad consume 100\% of threads
			\item[14] \qquad\qquad \textit{threads} $\xleftarrow{}$ number of consumed threads
			\item[15] \qquad\qquad \textit{if} $($\textit{threads} $>2^X+1)$
			\item[16] \qquad\qquad\qquad break the while loop
			\item[17] \qquad\qquad packet $\xleftarrow{}$ \textit{decimalToBinary(threads)}
			\item[18] \qquad\qquad Release all the threads
			\item[19] \}\}
		\end{enumerate}
		
		\item \textbf{Change Roles.}
		\begin{enumerate}
			\item[1] \textit{if} $($isSender$)\{$
			\item[2] \qquad isSender $\xleftarrow{}$ false
			\item[3] \qquad Go To Step~\ref{item:msg}
			\item[4] $\}$ \textit{else} $\{$
			\item[5] \qquad isSender $\xleftarrow{}$ true
			\item[6] \qquad Go To Step~\ref{item:msg}
			\item[7] $\}$
		\end{enumerate}
	\end{enumerate}
\end{algorithm} 

\subsection{Edge Cases.}
One edge case is sending a packet that its decimal equivalent is zero. It makes
an issue, because for sending this packet, the sender does not 
need to release any thread and the 
receiver cannot observe changes in the number of free threads. 
Instead, in this case, we decided to send $2^X$ (The maximum value of
each packet plus one). For example, if the size of each packet is X=7, 
for sending 0000000, the sender releases 128 threads (sends 10000000). 
TO DO ...

\subsection{Case Study 1: WebSocket pool}

\begin{itemize}
	\item[-] what is websocket
	\item[-] Talking about chromium internals. 
	\item[-] what is the issue
\end{itemize}

\subsection{Case Study 2: Server Sent Event (SSE) pool}

\begin{itemize}
	\item[-] what is sse
	\item[-] Talking about chromium internals. 
	\item[-] what is the issue
\end{itemize}


==> scraps/browser-engines.tex <==
\begin{table}[t]
  \begin{center}
    \begin{tabular}{ll}
      \toprule
        Engine    & Browsers \\
      \midrule
        Chromium  & Brave, Chrome, Edge \\
        Gecko     & Firefox, Tor Browser Bundle \\
        WebKit    & Safari \\
      \bottomrule
    \end{tabular}
  \end{center}
  \caption{Summary of which popular browsers use which underlying browser
    engine, in alphabetical order.}
  \label{table:browser-engines}
\end{table}


==> scraps/evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}


\subsection{comparing browsers}
\begin{itemize}
	\item vulnerabilities in each browser.
	\item vulnerability in the private mode.
	\item the size of thread pool in each browser.
	\item summeraizing everything into table~\ref{tab:browsers}
\end{itemize}

\begin{table}[t]
	\centering
	\caption{Compare the vulnerability in different browsers}
	\begin{tabular}{lccc}
		\hline
		Browsers&
		Vulnerable&
		Private Mode&
		...\\
		\hline
		
		%Row 1
		\cellcolor{Gray}Chrome& 
		\cellcolor{Gray}\fullcirc& 
		\cellcolor{Gray}\emptycirc& 
		\cellcolor{Gray}\\
		
		%Row 2
		Edge&   
		\fullcirc& 
		\emptycirc& 
		\\
		
		%Row 3
		\cellcolor{Gray}Firefox& 
		\cellcolor{Gray}\fullcirc& 
		\cellcolor{Gray}\fullcirc& 
		\cellcolor{Gray}\\
		
		%Row 4
		Brave&   
		\fullcirc& 
		\emptycirc& 
		\\
		
		%Row 5
		\cellcolor{Gray}Safari& 
		\cellcolor{Gray}\fullcirc& 
		\cellcolor{Gray}\emptycirc& 
		\cellcolor{Gray}\\
		
		%Row 6
		TOR Browser&   
		\fullcirc& 
		\fullcirc& 
		\\
		
		%Row 8
		\cellcolor{Gray}Opera& 
		\cellcolor{Gray}\fullcirc& 
		\cellcolor{Gray}\emptycirc& 
		\cellcolor{Gray}\\
		\hline
		
	\end{tabular}
	\label{tab:browsers}
\end{table}

\subsection{Websockets in the wild}

\textbf{Crawler.}
\begin{itemize}
	\item Talking about our methodology
	\item We use chrome histograms
	\item The data that we collect from each website
	\item The implementation details of the crawler
\end{itemize}

\textbf{Results of crawling.}

\begin{itemize}
	\item The set of websites that we crawl
	\item The number of websites that use websockets
	\item A plot that shows the distribution of using websockets 
	\item How many of them close a websocket (make noise)
\end{itemize}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.4\textwidth]{figures/test.png}
	\caption{Replace this with the distribution of the number of 
		websockets used by websites}
	\label{fig:distribution}
\end{figure}

\subsection{Attack throughput.}

% Raw data is available here:
% https://docs.google.com/spreadsheets/d/1kXU9yy19LZvoB7ocr7-h8wv7W0A7sefO9wkqGIzZyZA/edit#gid=0

At the beginning of the protocol, there is a fix processing time (not in 
the order of data length) for the first and second step. Thus, for measuring the
throughput we just focus on the Message Exchange step.

For measuring the throughput in a real world scenario, we open cnn.com and nytimes.com
using selenium and inject our attack script into them. Our script sends five packets
(each packet has seven bits) from one website to the other one. We repeated this process
50 times for each browser and measure the timing data of each step. 

The median of \emph{Signal} and \emph{Synchronize} steps are shown in the 
table~\ref{tab:initDelay}. While Firefox's cap is 56 less than Chromium based browsers' cap,
it is slower than them. Throughput is shown in the Figure~\ref{fig:troughput}. Chromium based
browsers are faster with a throughput around 0.75 bits per second.


\begin{table}[t]
	\centering
	\caption{Signal and Synchronization delay in seconds}
	\begin{tabular}{lcc}
		\hline
		Browsers&
		Signal&
		Synchronize\\
		\hline
		
		%Row 1
		\cellcolor{Gray}Chrome& 
		\cellcolor{Gray}39& 
		\cellcolor{Gray}21\\
		
		%Row 2
		Edge&   
		39& 
		18\\
		
		%Row 3
		\cellcolor{Gray}Firefox& 
		\cellcolor{Gray}44& 
		\cellcolor{Gray}24\\
		
		%Row 4
		Brave&   
		37& 
		21\\
		
		%Row 5
		\cellcolor{Gray}Safari& 
		\cellcolor{Gray}& 
		\cellcolor{Gray}\\
		
		%Row 6
		TOR Browser& 
		& 
		\\
		
		%Row 8
		\cellcolor{Gray}Opera& 
		\cellcolor{Gray}38& 
		\cellcolor{Gray}21\\
		\hline
		
	\end{tabular}
	\label{tab:initDelay}
\end{table}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.5\textwidth]{figures/throughput/throughput.eps}
	\caption{Each candle shows the throughput for each browser}
	\label{fig:troughput}
\end{figure}

==> scraps/prev_abstract.tex <==
\begin{abstract}

%Cross-site tracking is a critical problem on the Web that browser vendors are addressing with a range of approaches. Ensuring these protections are robust is critical to protect users. In this work weee

% ``Cross-site tracking,'' or a party linking a
% person's behavior across sites in a way unintended
% or unwanted by the individual, is a common privacy violation on the \Web{}. Browsers
% primarily protect users from ``cross-site tracking'' by
% blocking or partitioning third-party storage, thereby denying sites
% a common value to link different sessions.
% While blocking or partitioning third-party state makes
% tracking more difficult, there are well known
% ways trackers can reestablish identifiers that are unique-to-the-user and shared-across-sites. These
% include deriving stateless identifiers (i.e., browser fingerprinting)
% or manipulating micro-architectural implementation
% details (e.g., graphics caches, CPU caches, etc). Though
% sometimes effective, these attacks are increasingly limited by other
% browser and OS defenses.

% In this work, we discuss an understudied category of
% cross-site tracking attack we call \TechniqueName{} attacks.  \uTechniqueName{} attacks
% are unaffected by OS-level mitigations for micro-architectural
% attacks, and are robust against browser-level privacy protections. Forms of this attack
% work in all major browser engines, and we provide proof of concept \TechniqueName{}
% attacks that work in all popular browsers. We expect forms of the attack would
% be successful in any browser built on current versions of Chromium, Gecko or WebKit.

% Though some forms of this attack have been documented, this work furthers the
% state of browser privacy with the following contributions. First,
% we define a general category of attack that can be carried out against nearly any
% \LBU{} pool of page accessible resources. Second, we demonstrate
% that \TechniqueName{} attacks are practical, real world cross-site tracking mechanisms that
% can be exploited in all current popular browsers, and share our open source
% implementation.
% Third, and alarmingly, we show that in Gecko based-browsers, \TechniqueName{} attacks allow not
% only cross-site tracing, but \emph{cross-profile} tracking (\EG linking behavior
% across normal and private browsing windows). Fourth, we present strategies
% browser vendors can use to protect users from \TechniqueName{} attacks.


\end{abstract}

